Understanding Iterative Revision from Human-Written Text

Writing is, by nature, a strategic, adaptive, and more importantly, an iterative process. A crucial part of writing is editing and revising the text. Previous works on text revision have focused on defining edit intention taxonomies within a single domain or developing computational models with a single level of edit granularity, such as sentence-level edits, which differ from human's revision cycles. This work describes IteraTeR: the first large-scale, multi-domain, edit-intention annotated corpus of iteratively revised text. In particular, IteraTeR is collected based on a new framework to comprehensively model the iterative text revisions that generalize to various domains of formal writing, edit intentions, revision depths, and granularities. When we incorporate our annotated edit intentions, both generative and edit-based text revision models significantly improve automatic evaluations. Through our work, we better understand the text revision process, making vital connections between edit intentions and writing quality, enabling the creation of diverse corpora to support computational modeling of iterative text revisions.

==> conclusion.tex <==
\section{Discussions and Conclusions}

In this work, we take a few vital steps to bridge gaps in prior computational and cognitive science research to understand the complex process of text revision and its iterative nature, covering the broad spectrum of domains, granularities, edit intentions, and iterations that a process like this requires for a thorough and complete analysis.

Our new edit intention taxonomy generalizes to multiple domains, granularities, and revisions, enabling us to collect complex text editing annotations with crowdsourcing across these different dimensions. We collect, annotate and release \textsc{IteraTE}: a novel, large-scale, domain-diverse, annotated dataset of human editing actions. We release both the smaller, human-labeled and the larger, automatically-labeled dataset for further research. 

We analyze human-editing patterns and study their effects on text quality, both against existing standard metrics and also against subjective criteria along different dimensions. This provides crucial insights towards understanding the motivations and consequences of human revision patterns.

Finally, we computationally model the process using state-of-the-art text editing and text generation techniques and provide insights into the modeling challenges of the task. By analyzing the edits made by our text editing models and comparing them against human editing patterns and text quality metrics, we take a significant step in understanding and exposing the challenges to computationally model iterative text editing.

In future work, we aim to dive deeper into these limitations and challenges of computationally modeling the task, and develop a system that can perform end-to-end iterative revisions. The \textsc{IteraTE} dataset, the findings of our annotation study, our text editing models, and our human evaluations will collectively serve as a basis for future corpus development and computationally modeling Iterative Text Editing. 

==> tab/model_performances_small.tex <==
\begin{table}[t]
  \centering
  \small
  \begin{tabular}{@{}l@{\hskip 2mm}lcccc@{}}
    \toprule
    \textbf{Model} & \textbf{Dataset} & \textbf{SARI} & \textbf{DEL} & \textbf{ADD} & \textbf{KEEP}  \\
    \midrule
    \textsc{FELIX} & \textsc{human-raw} & 29.23 & 19.23 & 0.62 & 67.85\\
    \textsc{FELIX} & \textsc{human} & 30.65 & 20.26 & 0.99 & 70.71 \\
    \textsc{FELIX} & \textsc{full-raw} & 30.34 & 20.44 & 1.40 & 69.18 \\
    \textsc{FELIX} & \textsc{full} & \textbf{33.48} & \textbf{22.39} & \textbf{2.52} & \textbf{75.52}\\
    \midrule
    \midrule
    \textsc{T5} & \textsc{human-raw} & 32.19 & 6.75 & 1.61 & \textbf{88.19} \\
    \textsc{T5} & \textsc{human} & 32.26 & 8.16 & 0.93 & 87.69 \\
    \textsc{T5} & \textsc{full-raw} & 33.24 & 10.47 & 1.38 & 87.87 \\
    \textsc{T5} & \textsc{full} & \textbf{34.45} & \textbf{13.62} & \textbf{4.19} & 85.54 \\
    \midrule
    \textsc{BART} & \textsc{human-raw} & 33.20 & 9.81 & 3.58 & 86.20 \\
    \textsc{BART} & \textsc{human} & 34.77 & 13.43 & \textbf{5.91} & 84.97 \\
    \textsc{BART} & \textsc{full-raw} & 33.88 & 12.38 & 2.34 & \textbf{86.92} \\
    \textsc{BART} & \textsc{full} & \textbf{37.28} & \textbf{19.83} & 5.69 & 86.33 \\
    \midrule
    \textsc{Pegasus} & \textsc{human-raw} & 33.09 & 10.61 & 1.57 & 87.09 \\
    \textsc{Pegasus} & \textsc{human} & 34.43 & 13.26 & 2.89 & 87.14 \\
    \textsc{Pegasus} & \textsc{full-raw} & 34.67 & 13.93 & 2.36 & \textbf{87.53} \\
    \textsc{Pegasus} & \textsc{full} & \textbf{37.11} & \textbf{19.66} & \textbf{4.44} & 87.16\\
    \midrule
    Baseline & - & 29.47 & 0.0 & 0.0 & 88.42  \\
    \bottomrule
  \end{tabular}
  \caption{\label{tab:model-performances-sari}
  Model performances on the test set of \textsc{IteraTeR-human}.  Baseline refers to a no-edit baseline, where we simply use the input text as the output.
  }
\end{table}
